Multi-Attribute Open Set Recognition

Open Set Recognition (OSR) extends image classification to an open-world setting, by simultaneously classifying known classes and identifying unknown ones. While conventional OSR approaches can detect Out-of-Distribution (OOD) samples, they cannot provide explanations indicating which underlying visual attribute(s) (e.g., shape, color or background) cause a specific sample to be unknown. In this work, we introduce a novel problem setup that generalizes conventional OSR to a multi-attribute setting, where multiple visual attributes are simultaneously recognized. Here, OOD samples can be not only identified but also categorized by their unknown attribute(s). We propose simple extensions of common OSR baselines to handle this novel scenario. We show that these baselines are vulnerable to shortcuts when spurious correlations exist in the training dataset. This leads to poor OOD performance which, according to our experiments, is mainly due to unintended cross-attribute correlations of the predicted confidence scores. We provide an empirical evidence showing that this behavior is consistent across different baselines on both synthetic and real world datasets.

==> figures/tex/figure_cconf_ut_zappos.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/images/cconf_ut_zappos/cnn_semi_correlated.jpg}
    \label{fig:cconf_ut_zappos_softmax}
    \caption{Cross-attribute confidence scores on UT-Zappos using the MSP approach}
\end{figure}

==> tables/table_correlations_auroc_avg_real.tex <==
\begin{table*}[t]
\caption{AUROC Evaluation averaged from all attributes.}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}{c|ccc}
\Xhline{4\arrayrulewidth}
\multirow{2}{*}{Approach} & \multicolumn{3}{c}{UT-Zappos} \\ 
& $\mathcal{A}_c$ & $\mathcal{A}_s$ & $\bar{\mathcal{A}}$ \\ \hline
 MSP & $45.9$ & $66.5$ & $56.2$ \\
 MLS & $44.3$ & $68.6$ & $56.4$ \\  
 ARPL & $51.2$ & $65.1$ & $58.1$ \\
 ARPL+CS & $49.8$ & $72.2$ & $61.0$ \\
 \Xhline{4\arrayrulewidth}
\end{tabular}
\label{table:correlations_auroc_avg_real}
\end{table*}


% \begin{table*}[ht]
% \caption{OSCR Evaluation averaged from all attributes.}
% \centering
% \fontsize{9}{11}\selectfont
% \begin{tabular}{c|ccc}
% \Xhline{4\arrayrulewidth}
% \multirow{2}{*}{Approach} & \multicolumn{3}{c}{Color-Fashion} \\ 
% & $\mathcal{A}_1$ & $\mathcal{A}_2$ & $\bar{\mathcal{A}}$ \\ \hline
%  MSP & $43.9$ & $51.7$ & $47.8$ \\
%  ARPL & $38.3$ & $54.1$ & $46.2$\\
%  ARPL+CS & $42.3$ & $41.6$ & $42.0$ \\
%  MSL & $44.2$ & $53.0$ & $48.6$ \\ 
%  \Xhline{4\arrayrulewidth}
% \end{tabular}
% \label{table:correlations_oscr_avg_real}
% \end{table*}


==> tables/table_correlations_cg_hm_acc.tex <==
\begin{table*}[th!]
\caption{Harmonic Mean CG Accuracy}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{4\arrayrulewidth}
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Color-MNIST} & \multicolumn{3}{c|}{Colored-Objects} & \multicolumn{3}{c}{Scene-Objects} \\ %\hline
& UC & SC & C & UC & SC & C & UC & SC & C \\ \hline
 ARPL           & $0.944$      & $0.409$                & $0.210$    & $0.597$                    & $0.297$                              & $0.176$                  & $0.270$                    & $0.199$                              & $0.146$                  \\
 ARPL-Ind       & $0.991$      & $0.499$                & $0.209$    & $0.753$                    & $0.365$                              & $0.179$                  & $0.369$                    & $0.252$                              & $0.151$                  \\
 CNN            & $0.979$      & $0.002$                & $0.001$    & $0.723$                    & $0.014$                              & $0.000$                  & $0.298$                    & $0.019$                              & $0.001$                  \\
 CNN-Ind        & $0.988$      & $0.192$                & $0.010$    & $0.749$                    & $0.200$                              & $0.001$                  & $0.351$                    & $0.183$                              & $0.060$                  \\
 CNNOpenMax     & $0.973$      & $0.015$                & $0.004$    & $0.692$                    & $0.019$                              & $0.012$                  & $0.281$                    & $0.056$                              & $0.023$                  \\
 LabelEmbedPlus & $0.961$      & $0.116$                & $0.010$    & N/A                        & N/A                                  & N/A                      & N/A                        & N/A                                  & N/A                      \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\label{table:correlations_cg_hm_acc}
\end{table*}


==> tables/table_correlations_cg_seen_acc.tex <==
\begin{table*}[th!]
\caption{Seen CG Accuracy}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{4\arrayrulewidth}
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Color-MNIST} & \multicolumn{3}{c|}{Colored-Objects} & \multicolumn{3}{c}{Scene-Objects} \\ %\hline
& UC & SC & C & UC & SC & C & UC & SC & C \\ \hline
 ARPL           & $0.944$      & $0.419$                & $0.211$    & $0.597$                    & $0.308$                              & $0.185$                  & $0.270$                    & $0.201$                              & $0.151$                  \\
 ARPL-Ind       & $0.991$      & $0.507$                & $0.209$    & $0.753$                    & $0.373$                              & $0.182$                  & $0.369$                    & $0.250$                              & $0.140$                  \\
 CNN            & $0.979$      & $0.996$                & $1.000$    & $0.723$                    & $0.899$                              & $1.000$                  & $0.298$                    & $0.484$                              & $0.747$                  \\
 CNN-Ind        & $0.988$      & $0.997$                & $1.000$    & $0.749$                    & $0.882$                              & $1.000$                  & $0.351$                    & $0.514$                              & $0.431$                  \\
 CNNOpenMax     & $0.973$      & $0.986$                & $0.996$    & $0.692$                    & $0.724$                              & $0.965$                  & $0.281$                    & $0.351$                              & $0.639$                  \\
 LabelEmbedPlus & $0.961$      & $0.926$                & $0.999$    & N/A                        & N/A                                  & N/A                      & N/A                        & N/A                                  & N/A                      \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\label{table:correlations_cg_seen_acc}
\end{table*}


==> tables/table_correlations_cg_unseen_acc.tex <==
\begin{table*}[th!]
\caption{Unseen CG Accuracy}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{4\arrayrulewidth}
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Color-MNIST} & \multicolumn{3}{c|}{Colored-Objects} & \multicolumn{3}{c}{Scene-Objects} \\ %\hline
& UC & SC & C & UC & SC & C & UC & SC & C \\ \hline
 ARPL           & $-1.000$     & $0.400$                & $0.213$    & $-1.000$                   & $0.288$                              & $0.168$                  & $-1.000$                   & $0.202$                              & $0.149$                  \\
 ARPL-Ind       & $-1.000$     & $0.492$                & $0.212$    & $-1.000$                   & $0.360$                              & $0.177$                  & $-1.000$                   & $0.257$                              & $0.178$                  \\
 CNN            & $-1.000$     & $0.001$                & $0.000$    & $-1.000$                   & $0.007$                              & $0.000$                  & $-1.000$                   & $0.010$                              & $0.001$                  \\
 CNN-Ind        & $-1.000$     & $0.109$                & $0.005$    & $-1.000$                   & $0.114$                              & $0.001$                  & $-1.000$                   & $0.112$                              & $0.033$                  \\
 CNNOpenMax     & $-1.000$     & $0.007$                & $0.002$    & $-1.000$                   & $0.010$                              & $0.006$                  & $-1.000$                   & $0.030$                              & $0.012$                  \\
 LabelEmbedPlus & $-1.000$     & $0.062$                & $0.005$    & N/A                        & N/A                                  & N/A                      & N/A                        & N/A                                  & N/A                      \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\label{table:correlations_cg_unseen_acc}
\end{table*}


==> tables/table_correlations_close_acc_0.tex <==
\begin{table*}[ht]
\caption{Close Set Accuracy for Factor 0 (Shape/Foreground)}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{4\arrayrulewidth}
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Color-MNIST} & \multicolumn{3}{c|}{Colored-Objects} & \multicolumn{3}{c}{Scene-Objects} \\ %\hline
& UC & SC & C & UC & SC & C & UC & SC & C \\ \hline
 ARPL           & $0.945$      & $0.418$                & $0.214$    & $0.604$                    & $0.294$                              & $0.171$                  & $0.405$                    & $0.346$                              & $0.298$                  \\
 ARPL-Ind       & $0.989$      & $0.502$                & $0.212$    & $0.767$                    & $0.368$                              & $0.175$                  & $0.525$                    & $0.394$                              & $0.308$                  \\
 CNN            & $0.917$      & $0.399$                & $0.220$    & $0.734$                    & $0.368$                              & $0.181$                  & $0.446$                    & $0.343$                              & $0.302$                  \\
 CNN-Ind        & $0.956$      & $0.466$                & $0.218$    & $0.754$                    & $0.427$                              & $0.181$                  & $0.503$                    & $0.385$                              & $0.276$                  \\
 CNNOpenMax     & $0.913$      & $0.397$                & $0.238$    & $0.712$                    & $0.260$                              & $0.181$                  & $0.433$                    & $0.288$                              & $0.288$                  \\
 LabelEmbedPlus & $0.880$      & $0.375$                & $0.215$    & N/A                        & N/A                                  & N/A                      & N/A                        & N/A                                  & N/A                      \\
 \Xhline{4\arrayrulewidth}
\end{tabular}
\label{table:correlations_close_acc_0}
\end{table*}


==> tables/table_correlations_close_acc_1.tex <==
\begin{table*}[ht]
\caption{Close Set Accuracy for Factor 1 (Color/Background)}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{4\arrayrulewidth}
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Color-MNIST} & \multicolumn{3}{c|}{Colored-Objects} & \multicolumn{3}{c}{Scene-Objects} \\ %\hline
& UC & SC & C & UC & SC & C & UC & SC & C \\ \hline
 ARPL           & $0.999$      & $0.999$                & $0.999$    & $0.994$                    & $0.994$                              & $0.994$                  & $0.671$                    & $0.580$                              & $0.514$                  \\
 ARPL-Ind       & $1.000$      & $0.999$                & $0.998$    & $0.994$                    & $0.996$                              & $0.995$                  & $0.714$                    & $0.641$                              & $0.564$                  \\
 CNN            & $0.999$      & $0.999$                & $0.998$    & $0.990$                    & $0.983$                              & $0.992$                  & $0.680$                    & $0.588$                              & $0.525$                  \\
 CNN-Ind        & $0.999$      & $0.999$                & $0.998$    & $0.995$                    & $0.993$                              & $0.993$                  & $0.672$                    & $0.625$                              & $0.400$                  \\
 CNNOpenMax     & $0.996$      & $0.990$                & $0.957$    & $0.978$                    & $0.940$                              & $0.956$                  & $0.668$                    & $0.515$                              & $0.509$                  \\
 LabelEmbedPlus & $0.999$      & $0.969$                & $0.976$    & N/A                        & N/A                                  & N/A                      & N/A                        & N/A                                  & N/A                      \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\label{table:correlations_close_acc_1}
\end{table*}


==> tables/table_correlations_close_acc_avg.tex <==
\begin{table*}[th!]
\caption{Average Close-Set accuracy from different dataset settings}
\centering
\fontsize{9}{11}\selectfont
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{4\arrayrulewidth}
\multirow{2}{*}{Approach} & \multicolumn{3}{c|}{Color-MNIST} & \multicolumn{3}{c|}{Colored-Objects} & \multicolumn{3}{c}{Scene-Objects} \\ %\hline
& UC & SC & C & UC & SC & C & UC & SC & C \\ \hline
 ARPL           & $0.972$      & $0.708$                & $0.607$    & $0.799$                    & $0.644$                              & $0.582$                  & $0.538$                    & $0.463$                              & $0.406$                  \\
 ARPL-Ind       & $0.994$      & $0.751$                & $0.605$    & $0.881$                    & $0.682$                              & $0.585$                  & $0.620$                    & $0.518$                              & $0.436$                  \\
 CNN            & $0.958$      & $0.699$                & $0.609$    & $0.862$                    & $0.676$                              & $0.587$                  & $0.563$                    & $0.465$                              & $0.413$                  \\
 CNN-Ind        & $0.978$      & $0.732$                & $0.608$    & $0.875$                    & $0.710$                              & $0.587$                  & $0.588$                    & $0.505$                              & $0.338$                  \\
 CNNOpenMax     & $0.954$      & $0.693$                & $0.597$    & $0.845$                    & $0.600$                              & $0.569$                  & $0.550$                    & $0.402$                              & $0.399$                  \\
 LabelEmbedPlus & $0.940$      & $0.672$                & $0.595$    & N/A                        & N/A                                  & N/A                      & N/A                        & N/A                                  & N/A                      \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\label{table:correlations_oscr}
\end{table*}

% \begin{table}[ht]
%     \centering
% \begin{tabular}{lllll}
% \hline
%                 & correlated & semi_correlated_12_36 & semi_correlated_12_36u & uncorrelated \\
%  ARPL           & $0.503$    & $0.938$               & $0.964$                & $0.998$      \\
%  CNN            & $0.586$    & $0.678$               & $0.680$                & $0.989$      \\
%  CNNOpenMax     & $0.566$    & $0.657$               & $0.670$                & $0.984$      \\
%  LabelEmbedPlus & $0.584$    & $0.687$               & $0.650$                & $0.985$      \\
% \hline
% \end{tabular}
% 	\caption{Close Acc DV.}
% 	\label{tab:correlations_close_acc}
% \end{table}
